An Empirical Investigation on the Challenges Faced by Women in the Software Industry: A Case Study

Addressing women's under-representation in the software industry, a widely recognized concern, requires attracting as well as retaining more women. Hearing from women practitioners, particularly those positioned in multi-cultural settings, about their challenges and and adopting their lived experienced solutions can support the design of programs to resolve the under-representation issue. Goal: We investigated the challenges women face in global software development teams, particularly what motivates women to leave their company; how those challenges might break down according to demographics; and strategies to mitigate the identified challenges. Method: To achieve this goal, we conducted an exploratory case study in Ericsson, a global technology company. We surveyed 94 women and employed mixed-methods to analyze the data. Results: Our findings reveal that women face socio-cultural challenges, including work-life balance issues, benevolent and hostile sexism, lack of recognition and peer parity, impostor syndrome, glass ceiling bias effects, the prove-it-again phenomenon, and the maternal wall. The participants of our research provided different suggestions to address/mitigate the reported challenges, including sabbatical policies, flexibility of location and time, parenthood support, soft skills training for managers, equality of payment and opportunities between genders, mentoring and role models to support career growth, directives to hire more women, inclusive groups and events, women's empowerment, and recognition for women's success. The framework of challenges and suggestions can inspire further initiatives both in academia and industry to onboard and retain women.

==> Tables/regression.tex <==
\begin{table}[!htb]
	\footnotesize
	\centering
	\caption{The linear regression models per each category of challenge with standardized coefficients showing how different factors influence the reporting of each category of challenge. The level of statistical significance is indicated with asterisks: (*) for p < .05, (**) for p < .01, and (***) for p < .001}
	\label{tab:regressionresults}
	\begin{tabular}{|l|l|l|}
		\toprule
		\hline
		Lack of Peer Parity
		 \hline
		\textbf{Coefficients}   & \textbf{Estimate} & \textbf{Pr(\textgreater{}|z|)} \\ \hline\hline
		(Intercept)             & 1.2743            & 0.0341 (*)                     \\ \hline
		\textbf{Age: 25 to 34 and Experience in SW Industry: Less than  years           & -4.504e+15            & <2e-16 (***)}                        \\ \hline
	
	\end{tabular}
\end{table}

==> Tables/survey_questions.tex <==

\begin{table*}[htb]
\centering
\caption{Survey Questions (excluding demographic questions)}
\label{tab:survey_questions}
\footnotesize
\begin{tabular}{l}
\hline
\toprule
\multicolumn{1}{c}{\cellcolor{gray!35}\textbf{Survey Questions}}                                                                                  \\ \hline\hline
S-1. Please tell us the major difficulties/challenges you face (as a woman) during your work at [company name] (Open Question)             \\ \hline
S-2. Can you tell us the reason(s) that caused any women you know to leave [company name] (Open Question)                                 \\ \hline
S-3. What would you recommend [company name] do to have more women?
\bottomrule
\end{tabular}
\end{table*}

==> not_used.tex <==
**** Method regression ****

\subsection{Quantitative Analysis}
\label{sec:method:quantitative}

To address RQ2, 
%We used descriptive statistics to rank attributes and regression modelling techniques to identify demographics that positively or negatively influence the reporting of each challenge
we used regression modeling techniques to identify demographics that have any relation and can perhaps influence the likelihood of a respondent to report each category of challenge, having the demographics as independent variables and each category of challenge as the dependent variable. We completed all analysis in the R Studio statistical software.

To check for collinearity among the explanatory variables in the regression models, we first checked for Variable Inflation Factors (VIF). A recommended practice is to remove any variables in the final model that have VIF scores $>5$ \cite{fox2015applied}. Based on the VIF scores, we selected the following variables to be part of the model: experience, tenure, age, country, marital status and living (or not) with children. The VIF scores of these variables were $<2$, signifying low collinearity among the variables.

%We also used descriptive statistics to summarize the survey responses and the demographics data ~\cite{wohlin2015towards}. 

**** Results regression ****

We used multiple linear regression models to evaluate the influence of demographics in the reported challenges, as discussed in Section~\ref{sec:method:data_analysis}. The negative coefficients indicate that an increase in these factors is linked with a decrease in the likelihood of perceiving the challenge. We only display statistically significant results
(p < 0.05) in our tables and in the text we provide coefficients in parentheses. Our analysis is based exclusively on the data from this study's survey.

We found relation between the challenges of \textsc{Peer parity}, \textsc{Work-Life Balance Issues} and \textsc{Glass Ceiling} and demographics, as we present below. Sexism, Impostor Syndrome, Prove-it-Again, Maternal Wall, Lack of Recognition had no relation with demographics' data.

\subsubsection{Lack of Peer Parity: Younger and new in company}

The results from linear regression model using \textsc{peer parity} as the dependent variable suggested the interaction of age and tenure (years in company) are related with the challenge. Women from our sample who are working in the company for less than 3 years, and age less than 34 years old might report this challenge. While that, women with more than 45 years old, even having the same recent tenure, might not report this challenge.

%\input{Tables/regression}

age: $<$ 34 years old and tenure: $<$ 3 years (Positive estimate: 5.629e+15, p$<$2e-16 ***)
age: $>$ 45 years old and tenure: $<$ 3 years (Negative estimate: -1.238e+16, p$<$2e-16 ***)
anova of age with tenure: p=0.001084 **
    
\subsubsection{Work-life Balance issues: Women who live with children, specially when having more than 10 years in the company}

The results from linear regression model using \textsc{work-life balance issues} as the dependent variable suggested that living with children is a factor related with reporting this challenge, yet more when also working at the company for more than 10 years. While that, women who live with children but are working at the company for less than 3 years might not report this challenge.
    
havechildren: yes (Estimate 4.504e+15, p$<$2e-16 ***)
    anova of havechildren (p=0.01798 *)

tenure: $>$ 10 years and havechildren: yes (Estimate: 1.351e+16, p$<$2e-16 ***)
tenure: $<$ 3 years and havechildren: yes (Estimate: -1.059e+10, p$<$2e-16 ***)
    anova of tenure with havechildren (p$<$2.2e-16 ***)

\subsubsection{Glass Ceiling: Older women who are working in company for more than 10 years and younger women from India}

The results from linear regression model using \textsc{glass ceiling} as the dependent variable suggested the interactions of age with tenure (years in company) and age with country are related with the challenge. Women from our sample who have more than 45 years old and are working in the company for more than 10 years, and women from India who age less than 34 years old might report this challenge.

age: $>$ 45 years old and tenure: $>$ 10 years (Estimate: 3.965e+15, p$<$2e-16 ***)
    anova of age and tenure: p=0.001063 **

age: $<$ 34 years old and country: India (Estimate: 1.182e+16, p$<$2e-16 ***)
    anova of age and country: p=0.040753 *
    
    %Research is taking strides to understand the impact of lack of diversity within software development teams: challenges in the pipeline such as recruitment and education~\cite{clark2005women}, unconscious bias within organizations and online technology communities~\cite{reuben2014stereotypes,vasilescu2014gender}, and also how to design more inclusive software that is suitable for diverse learning and interaction styles\cite{burnett2016finding}.
